SonarSnoop: Active Acoustic Side-Channel Attacks

We report the first active acoustic side-channel attack. Speakers are used to emit human inaudible acoustic signals and the echo is recorded via microphones, turning the acoustic system of a smart phone into a sonar system. The echo signal can be used to profile user interaction with the device. For example, a victim's finger movements can be inferred to steal Android phone unlock patterns. In our empirical study, the number of candidate unlock patterns that an attacker must try to authenticate herself to a Samsung S4 Android phone can be reduced by up to 70% using this novel acoustic side-channel. Our approach can be easily applied to other application scenarios and device types. Overall, our work highlights a new family of security threats.

==> acoustics_not_used_anymore_.tex <==
% !TEX root = main.tex
\section{Movement Detection through Acoustics}\label{sec:movedetection}
\subsection{Overview}\label{subsec:acousticoverview}

Information from acoustic channel can be used to detect human behaviours. In this paper, we focus on a certain area of human behaviours which is movement. Detecting human body movement through the properties of acoustic signal is not completely novel~\cite{ShyamnathFingerIO,WangLLAP,YunStrata}, but our work exploits the security implication of this technique with a common real life scenario. We exploit the detection capability of acoustic signal to break the well-known defense mechanism - unlock patterns. From this perspective, we explore the feasibility of acoustic side-channel analysis. There are some existing research using sound data recorded by microphones to reveal keystrokes on mobile devices~\cite{SashankMicandGyro}. However, there is a big difference between our work and their work. This difference is that they use sensors to passively receive acoustic signals, but we use acoustic signal in a proactive way.

To use an active acoustic side-channel analysis method, we built a sonar system to send sound waves actively, then we analyzed the echo recorded to infer what movements are like. The principle is this: sound wave can be reflected by objects in the way of its travel path. If these objects keep moving within a period of time, some physical features of the echoes reflected by these moving objects can reveal information about the movement. The physical features are related to the properties of sound wave, such as Doppler effect, phase change and echo profile change~\cite{WangLLAP, ShyamnathFingerIO,YunStrata}. We choose echo profile as the property of sound wave to be analyzed as it is effective and intuitive. Echo profile can be generated through the correlation calculation between the acoustic signal actively sent by us and the echoes reflected by moving objects to microphones. Thus, we need to send a certain type of signal which has a good correlation property.

\subsection{Introducing OFDM}
\label{subsec:OFDM}
 \ac{OFDM} is a well-known modulation technique widely used in modern wireless systems as powerline networks, Wi-Fi and \ac{LTE}. \ac{OFDM} is a special form of \ac{FDM} by which a total bandwidth is divided into several non-overlapping frequency bands, and each of them is used to transmit different signals. The difference between \ac{OFDM} and normal \ac{FDM} is that the former requires all carrier signals are orthogonal to each other. We choose to send \ac{OFDM} signal, because the autocorrelation property of \ac{OFDM} signal is good~\cite{ShyamnathFingerIO}. 

To compose \ac{OFDM} signal, frequency bandwidth needs to be divided into a series of subcarriers each of which has a fixed bandwidth. For instance, the bandwidth is divided into N subcarriers and the n$^{th}$ subcarrier is used to transmit the data bit X$_n$, then we apply \ac{IFFT} to transform these data bits into N time-domain samples which will be sent by a transmitter (they should be real number), i.e.,

\begin{align*}
\textbf{x}_{k} = \sum_{n=0}^{N-1}\textbf{X}_ne^{i2\pi kn / N}\quad k=0 \  to \  N-1
\end{align*}

\subsection{Using acoustics as the side channel}

Side-channel attack means an attack trying to break the system through exploiting the information leaked via the physical implementation of the system. This is quite a big research area, and it contains several categories the number of which is highly possible to keep growing in the future. Side-channel analysis is widely studied in security area as it can often leak some unexpected but interesting information without alerting users. Besides this, new kinds of side-channel always keep emerging. There already exists many research work about using side-channel attack to reveal cryptographic keys and user PIN code, etc. However, there are only few papers trying to break security defence on smart devices using acoustic channel. \cite{SashankMicandGyro} infer users' unlock PINs and which keystrokes users have typed in on their phone screen by combining the sensing data of gyroscope sensor and microphones of a smartphone, but they use acoustic signal passively. To our best knowledge, there is no prior work about taking advantages of the detection capability of sound wave actively to reveal security relevant information on a daily-used mobile device. Our work is pioneering in this area.  



==> countermeasures.tex <==
Active acoustic side-channel is a new threat. It can violate people's information security severely. Countermeasures against this new acoustic side-channel can be implemented from four perspectives: hardware defence, \ac{OS} defence, application defence and centralized censorship defence. Please note that we try to avoid countermeasures which requires users' efforts too much.

\paragraph{Hardware Defence} It's not realistic to forbid the use of speakers and microphones of a devices or expect users to disable them intentionally. However, a dedicated anti-snooping instrument capable of jamming acoustic signals of inaudible frequency range is an option. Nandakumar et al. proposed similar idea about jamming signals in the inaudible range~\cite{ShyamnathCovertband}. This device can simply jam acoustic signals across possible frequency in the inaudible range . Furthermore, microphones could be included with this device to achieve jamming after sensing malicious acoustic signals. A smartphone can fulfil this responsibility.

\paragraph{\ac{OS} Defence} Hardware defence requires users' awareness of this new threat, and it needs extra electronic appliances. Countermeasures implemented on \ac{OS} level are more usable since they can be achieved without extra devices. \ac{OS} should query the status of speakers and microphones. Provided the system detects they are being accessed by some apps during phone unlock phase or during the launching of sensitive apps like banking apps, \ac{OS} should prohibit the access requested by other apps until unlock activity or the use of sensitive apps have finished.

\paragraph{Application Defence} There are two types of application level defence. First, as described in hardware defence, an app on another phone which finds acoustic signals in inaudible frequency range can jam the signal with noise. Second, sensitive applications (e.g. banking apps) can introduce noise to other sensors (e.g. microphones, accelerometer and gyroscope) to block potential side-channel attacks.

\paragraph{Centralized Censorship Defence} Application markets should be aware of this new acoustic side-channel possibility. They should censor the request list of applications. If any application requires the access to both speakers and microphones, a further check about in what frequency range these applications ask the speaker to work would be useful.



==> header_usenix.tex <==
\usepackage{graphicx}
\usepackage{subfig}

\usepackage[nolist]{acronym}

%\usepackage{flushend}

% Footnotes
\newcommand{\ethem}[1]{{\textbf{[IEB]}}\footnote{{\textbf{[Ethem]: }}#1}}
\newcommand{\utz}[1]{{\textbf{[UR]}}\footnote{{\textbf{[Utz]: }}#1}}
\newcommand{\jeff}[1]{{\textbf{[IEB]}}\footnote{{\textbf{[Jeff]: }}#1}}
\newcommand{\peng}[1]{{\textbf{[UR]}}\footnote{{\textbf{[Peng]: }}#1}}

%\newcommand{\ethem}[1]{{}}
%\newcommand{\utz}[1]{{}}
%\newcommand{\jeff}[1]{{}}
%\newcommand{\peng}[1]{{}}

\usepackage{siunitx}

\usepackage{booktabs}

\usepackage{caption}
\captionsetup{font=footnotesize}

\usepackage{xcolor}

\usepackage{enumitem}

% \usepackage[compact]{titlesec}
% \titlespacing{\section}{0pt}{5pt}{2pt}
% \titlespacing{\subsection}{0pt}{5pt}{2pt}
% \titlespacing{\subsubsection}{0pt}{5pt}{2pt}

\newcommand{\ur}[1]{{\color{red}{[Utz: #1]}}}
\newcommand{\ieb}[1]{{\color{red}{[Ethem: #1]}}}

==> related_work_backup.tex <==
% !TEX root = main.tex






To the best of our knowledge, this work is the first to explore the feasibility of active acoustic side-channel attack on stealing user information. Our case study is the first to present sonar-based active acoustic side-channel attack on an off-the-shelf mobile device to crack unlock patterns. This work belongs to the area of utilizing acoustic side-channel to get users' credential information. Related work can be divided into two categories. The first group includes work aiming to achieve device-free finger tracking via acoustics only using existing speaker and microphones in mobile devices, and the other category concludes acoustic side-channel attack. We will also introduce relevant non-acoustic side-channel analysis on mobile devices in this category.

\paragraph{Device-free Acoustic Finger Tracking}

Some work in \ac{HCI} area focusing on using acoustic signals for tracking human finger/hand movement without extra devices~\cite{ShyamnathFingerIO,WangLLAP,YunStrata}. These work tried to extract different physical features from echoes to infer the movement and location of finger or hand, and they aimed to achieve fairly high detecting accuracy. Nandakumar et al.~\cite{ShyamnathCovertband} used the sonar system to detect people's location, and linear or rhythmic motions in a 2D plane, and they can achieve this through wall. Our work is different from their work in three aspects. First, application scenarios are different. They did not study finger movement on the screen of the phone; second, they did not explore the the possibility of stealing sensitive data from users through their acoustic system; third, we create our novel automated analysis method. 

(NOT SURE IF WE NEED THIS PARAGRAPH)
When a user draws unlock patterns on a smartphone screen, there are different challenges for finger tracking. Firstly, the reflection paths are trickier because of the relative positions of the speakers, the microphones and our hand. If the front speaker was not enabled, ST and ET in Figure~\ref{fig:reflection_path} will disappear, which results in the invalidity of top microphone's echo data; secondly, 
to a single microphone, moving direction of a finger may be opposite to that of the palm because the relative position of our hands and the microphone. Therefore, echoes captured by the microphone represent a complex situation. We overcome this two issue through studying acoustic signal reflection path.



\paragraph{Relevant Side-channel Analysis Exposing User Information}

Obtaining information via acoustic side-channel is not new. However, most of them utilize acoustic signals passively by only listening to signals. We classified them as two groups. 

First, some work present attacks based on acoustic side-channel to obtain data indirectly. Backes et al.~\cite{BackesAcousticPrinters} achieved recovering the content printed by a dot-matrix printer through the sound it made. Faruque et al.~\cite{FaruqueAcoustic3DPrinter} explored to reconstruct the object printed by a 3D printer through the sound emitted. Hojjati et al.~\cite{HojjatiSideChannelFactory} demonstrate attacks on a 3D printer and a CNC mill using audio and magnetometer data. There are more work in this area~\cite{BelikovetskyDetecting,ChhetriConfidentiality}. Toreini et al.~\cite{ToreiniAcousticEnigma} decoded the keys pressed on an Enigma machine by analysing the sound. Genkin et al.~\cite{GenkinRSAAcoustic} demonstrated breaking full 4096-bit RSA keys using acoustic signals generated by the computer. 

The other group study recovering keystrokes on physical or virtual keyboard via acoustics.  Cai et al.~\cite{CaiSensorSniffing} did a survey to explore the potential attacks using microphones. Asonov et al.~\cite{Asonovkeyboard} first presented using acoustic attack to classify different key presses on a physical keyboard. Zhuang et al.~\cite{ZhuangKeyboard} further improved this work. Berger et al.~\cite{BergerDictionary} presented a dictionary attack based on keyboard acoustic emanations. Compagno et al.~\cite{CompagnoAcousticEavesdropping} realized inferring text typed on keyboard through the acoustic signal captured via Skype chat. Liu et al.~\cite{LiuSnooping} used two microphones on a smartphone to inference presses on a keyboard. Zhu et al.~\cite{ZhuContextfreeattacks} showed several context-free attacks on keyboard. Narain et al.~\cite{SashankMicandGyro} used gyroscope and microphones on a mobile phone to predict keystrokes on the virtual keyboard of a smartphone, we will discuss this work later. 


Some work applied side-channel analysis to get PINs or patterns entered by users on mobile devices. These side-channels include oil residues on the screen~\cite{AvivSmudge}, readings from accelerometer sensors~\cite{AvivAccelerometer}, data from microphones together with gyroscopes~\cite{SashankMicandGyro}, etc. 

Aviv et al.~\cite{AvivSmudge} estimated the possibility of extracting smudges, then did a initiatory analysis of guessing patterns according to the information coming from the smudges. 

Aviv et al.~\cite{AvivAccelerometer} used readings from accelerometer as a side-channel data to unveil users' input PIN numbers and graphical patterns. They implemented a dictionary attack. After collecting data, they broke the pattern data into individual swipes and the PIN data into separate touches, based on which they trained their machine learning model, then they used this dictionary to predict each swipe and touch of the patterns and PIN tested, then combined them to guess what patterns or PINs they are. This is similar to our D1 decision making strategy. However, the performance of their method will drop significantly when using dictionary attack, especially when training data and testing data come from different users.

Narain et al.~\cite{SashankMicandGyro} used data from gyroscope and microphones on mobile devices to predict the keystroke by users. Ye et al.~\cite{ZhengWangCrackingAndroidPattern} presents a video-based attack which can be launched by an attack 2 meters away from the victim covertly, they can break 95\% of the patterns in five attempts. Their work is based on mature computer-vision techniques, and there are antecedent work about using video-based attack to break PIN password~\cite{ShuklaVideoPIN}. Compared to their work, the working mechanism is different, and our attack is even more covert and automatic than \cite{ZhengWangCrackingAndroidPattern} since we do not need to film the finger movement near the victim. 

[Peng: I deleted the Android Pattern Lock Analysis]


